The Computation of Approximate Generalized Feedback Nash Equilibria

We present the concept of a Generalized Feedback Nash Equilibrium (GFNE) in dynamic games, extending the Feedback Nash Equilibrium concept to games in which players are subject to state and input constraints. We formalize necessary and sufficient conditions for (local) GFNE solutions at the trajectory level, which enable the development of efficient numerical methods for their computation. Specifically, we propose a Newton-style method for finding game trajectories which satisfy necessary conditions for an equilibrium, which can then be checked against sufficiency conditions. We show that the evaluation of the necessary conditions in general requires computing a series of nested, implicitly-defined derivatives, which quickly becomes intractable. To this end, we introduce an approximation to the necessary conditions which is amenable to efficient evaluation, and in turn, computation of solutions. We term the solutions to the approximate necessary conditions Generalized Feedback Quasi-Nash Equilibria (GFQNE), and we introduce numerical methods for their computation. In particular, we develop a Sequential Linear-Quadratic Game approach, in which a LQ local approximation of the game is solved at each iteration. The development of this method relies on the ability to compute a GFNE to inequality- and equality-constrained LQ games, and therefore specific methods for the solution of these special cases are developed in detail. We demonstrate the effectiveness of the proposed solution approach on a dynamic game arising in an autonomous driving application.

==> commented_out.tex <==
% One approach to algorithmically finding a GFNE trajectory is to find a solution satisfying \cref{eq:foncs} for stage $t=1$, and checking if it additionally satisfies the conditions outlined in \cref{thm:sufficiency}. Unfortunately the evaluation of the conditions \cref{eq:foncs} requires being able to evaluate $\pi_s(x_s)$ as well as $\nabla_{x_s} \pi_s(x_s)$, for which explicit forms are generally unavailable. For this reason, we introduce an approximation to an exact GFNE, which we denote a Generalized Feedback Quasi-Nash Equilibrium (GFQNE). Associated with a GFQNE are the policies $\hat{\pi_t}(x_t)$.

% \begin{definition}[GFQNE]
% A Generalized Feedback Quasi-Nash Equilibrium for the subgame starting at stage $t$ from state $x_t$ is defined in terms of the following Generalized Nash Equilibrium problems and corresponding policies. For stage $t=T$, we have that

% \begin{equation}
%     \label{eq:gqn_problem_T}
%     \hat{\pi}_T^i(x_T) := \pi_T^i(x_T),
% \end{equation}
% and for all other stages $t\in\{1,...,T-1\},$ we have that
% % \begin{subequations}
% % \label{eq:gqn_problem_t}
% % \begin{alignat}{3}
% %     \hat{\pi}_t^i(x_t) := \tilde{u}^i_t = \underset{u_t^i }{\textrm{\emph{arg}}} \underset{\substack{u_{t:T}^i,\\
% %     \tilde{u}^{-i}_{t+1:T},\\
% %     x_{t+1:T+1} \\
% %     \Lambda_{t+1}}}
% %     {\textrm{\emph{min}}}\ 
% %         &\sum_{s=t}^T l_s^i(x_s,u_s^i, \tilde{u}_s^{-i}) + l_{T+1}^i(x_{T+1}) 
% %     \\
% %     \textrm{s.t.} \ \ \ \ 
% %      & 0 \in \begin{bmatrix} x_{t+2:T+1}  \\ u^i_{t+1:T} \\ \tilde{u}^{-i}_{t+1:T} \\ \Lambda_{t+1} \end{bmatrix} - \Gamma_{t+1}(x_{t+1}) \label{eq:generalized_constraints} \\
% %     &0 = x_{t+1} - f(x_t,u_t^i, \tilde{u}_t^{-i}), \\
% %     % \begin{bmatrix} u_t^i \\ \vdots  \\ u_{T}^i  \end{bmatrix} &\in \underset{u_{t:T}^i}{\text{\emph{argmin}}} \sum_{s=t}^T\left\lVert e_s^i(x_s,u^i_s,\tilde{u}_s^{-i}) \right\rVert + \left\lVert e_{T+1}^i(x_{T+1}) \right\rVert  \label{eq:argmin_t}
% %     & 0 = h_t^i(x_t,u_t^i, \tilde{u}_t^{-i}) \\
% %     & 0 \leq g_t^i(x_t,u_t^i, \tilde{u}_t^{-i})
% % \end{alignat}
% % \end{subequations}

%  \begin{subequations}
% \label{eq:gqn_problem_t}
% \begin{alignat}{3}
%     \hat{\pi}_t^i(x_t) := \tilde{u}^i_t = \underset{u_t^i }{\textrm{arg}} \underset{\substack{u_{t:T}^i,\\
%     \tilde{u}^{-i}_{t+1:T},\\
%     x_{t+1:T+1}}}{\textrm{min}}\ 
%         &\sum_{s=t}^T l_s^i(x_s,u_s^i, \tilde{u}_s^{-i}) + l_{T+1}^i(x_{T+1}) 
%     \\
%     \textrm{s.t.} \ \ \ \ 
%      & 0 \in (u^i_s, \tilde{u}^{-i}_s) - \Gamma_s(x_s), \ &&s\in\mathbf{T_{t+1}} \label{eq:generalized_constraints} \\
%     &0 = x_{s+1} - f(x_s,u_t^i, \tilde{u}_s^{-i}), \ &&s\in\mathbf{T_t} \\
%     % \begin{bmatrix} u_t^i \\ \vdots  \\ u_{T}^i  \end{bmatrix} &\in \underset{u_{t:T}^i}{\text{\emph{argmin}}} \sum_{s=t}^T\left\lVert e_s^i(x_s,u^i_s,\tilde{u}_s^{-i}) \right\rVert + \left\lVert e_{T+1}^i(x_{T+1}) \right\rVert  \label{eq:argmin_t}
%     & 0 = h_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     & 0 \leq g_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     & 0 = h^i_{T+1}(x_{T+1}) \\
%     & 0 \leq g^i_{T+1}(x_{T+1})
% \end{alignat}
% \end{subequations}

% \end{definition}

% The point-to-set mappings $\Gamma_t$, $t\in\mathbf{T}$, are defined to be the sets of all control variables such that there exist primal and dual variables satisfying the first-order necessary conditions of the generalized Nash Equilibrium problems corresponding to the policies $\hat{\pi}_{t}$ evaluated at $x_{t}$. In particular,  $\Gamma_s(x_t)$ is the set of all $u_t$ such that there exist variables satisfying \cref{eq:qfoncs}, as shown below.
% \begin{subequations}
% \label{eq:gqn_problem_t}
% \begin{alignat}{3}
%     \hat{\pi}_t^i(x_t) := \tilde{u}^i_t = \underset{u_t^i }{\textrm{arg}} \underset{\substack{u_{t:T}^i,\\
%     \tilde{u}^{-i}_{t+1:T},\\
%     x_{t+1:T+1}}}{\textrm{min}}\ 
%         &\sum_{s=t}^T l_s^i(x_s,u_s^i, \tilde{u}_s^{-i}) + l_{T+1}^i(x_{T+1}) 
%     \\
%     \textrm{s.t.} \ \ \ \ 
%      & 0 \in \tilde{u}^{-i}_s - \Gamma^{-i}_s(x_s,\mathbf{z_s}), \ &&s\in\mathbf{T_{t+1}} \label{eq:generalized_constraints} \\
%     &0 = x_{s+1} - f(x_s,u_t^i, \tilde{u}_s^{-i}), \ &&s\in\mathbf{T_t} \\
%     % \begin{bmatrix} u_t^i \\ \vdots  \\ u_{T}^i  \end{bmatrix} &\in \underset{u_{t:T}^i}{\text{\emph{argmin}}} \sum_{s=t}^T\left\lVert e_s^i(x_s,u^i_s,\tilde{u}_s^{-i}) \right\rVert + \left\lVert e_{T+1}^i(x_{T+1}) \right\rVert  \label{eq:argmin_t}
%     & 0 = h_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     & 0 \leq g_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     & 0 = h^i_{T+1}(x_{T+1}) \\
%     & 0 \leq g^i_{T+1}(x_{T+1})
% \end{alignat}
% \end{subequations}

% \begin{subequations}
% \label{eq:gqn_problem_t}
% \begin{alignat}{3}
%     \hat{\pi}_t^i(x_t) := \tilde{u}^i_t = \underset{u_t^i }{\textrm{arg}} \underset{\substack{u_{t:T}^i,\\
%     \tilde{u}^{-i}_{t+1:T},\\
%     x_{t+1:T+1}}}{\textrm{min}}\ 
%         &\sum_{s=t}^T l_s^i(x_s,u_s^i, \tilde{u}_s^{-i}) + l_{T+1}^i(x_{T+1}) 
%     \\
%     \textrm{\emph{s.t.}} \ \ \ \ 
%     (u_s^i,\tilde{u}_s^{-i}) &= K_s(x_s), \ s\in\mathbf{T_{t+1}} \label{eq:qpolicy_foncs} \\
%     %  \tilde{u}^{-i}_s &= \pi^{-i}_s(x_s), \ s\in\mathbf{T_{t+1}} \label{eq:qpolicy_of_other_controls}\\
%     0 &= x_{s+1} - f(x_s,u_t^i, \tilde{u}_s^{-i}), \ s\in\mathbf{T_t} \\
%     u_t^i &\in \underset{u_{t}^i}{\text{argmin}} \left\lVert e_t^i(x_t,u^i_t,\tilde{u}_t^{-i},...,x_{T+1}) \right\rVert \label{eq:argmin_qt}
%     % & 0 = h_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     % & 0 \leq g_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     % & 0 = h^i_{T+1}(x_{T+1}) \\
%     % & 0 \leq g^i_{T+1}(x_{T+1})
% \end{alignat}
% \end{subequations}Here we have introduced
% Here the vector $\mathbf{z_s}$ is used to denote the set of all primal and dual variables associated with the sub-game at stage $s$:
% \begin{equation}
% \begin{aligned}
% \mathbf{z_s} &:= (u_s, \lambda_s, \mu_s, \gamma_s, \psi_{s+1}, x_{s+1}, \mathbf{z_{s+1}}) \\
% \mathbf{z_T} &:= (u_T, \lambda_T, \mu_T, \gamma_T, x_{T+1}, \lambda_{T+1}, \mu_{T+1}, \gamma_{T+1}).
% \end{aligned}
% \end{equation}

% The difference between \cref{eq:gn_problem_t} and \cref{eq:gqn_problem_t} is in the replacement of constraints \cref{eq:policy_of_other_controls} with \cref{eq:generalized_constraints}, which encode the requirement that every sub-game trajectory of the game satisfy first-order necessary conditions of the GFQNE for that sub-game, instead of requiring that the sub-game trajectories constitute a GFNE for the sub-game. 

% \begin{theorem}
% \label{thm:qfoncs} 
% For any solution $x_{t+1:T+1}^*, u_{t:T}^*$ of the problems \cref{eq:gqn_problem_T}/ \cref{eq:gqn_problem_t} at stage $t\in\mathbf{T}$, there exist associated multipliers such that the following conditions must hold:

% % The set $\Gamma_t(x_t) \subset (\mathcal{U}^1 \times ... \times \mathcal{U}^N)$, denoted to be the set of all such controls $u_t$ such that there exist multipliers $\{\lambda_s^i\in\mathbb{R}^n; \ s\in\mathbf{T_t}, \ i\in\mathbf{N}\}$, $\{\mu_s^i\in\mathbb{R}^{k^i_s}; \ s\in\mathbf{T_t^+}, \ i\in\mathbf{N}\}$, $\{\gamma_s^i\in\mathbb{R}^{j^i_s}; \ s\in\mathbf{T_t^+}, \ i\in\mathbf{N}\}$, and $\{\psi_s^i\in\mathbb{R}^{m^{-i}};\ s\in\mathbf{T_{t+1}}, \ i\in\mathbf{N}\}$ satisfying the first-order necessary conditions of \cref{eq:gqn_problem_t}, is expressed as the following:
% % \end{theorem}

% \begin{subequations}
%     \label{eq:qfoncs}
%     \begin{alignat}{3}
% %   & \mathrlap{\Gamma_t(x^*_t) := \Bigg\{ u^*_t \ : \ \exists x^*_{t+1:T+1}, u^*_{t+1:T}, \lambda_{t:T}, \mu_{t:T+1}, \gamma_{t:T+1}, \psi_{t+1:T}:} \\
% %   & \ \ \ \Updownarrow \\
% %   &\mathrlap{\exists \{x_{s+1}, s\in\mathbf{T_t}\}, \{u_s, s\in\mathbf{T_{t+1}}\}, \{\lambda_s, s\in\mathbf{T_t^+}\},} \\
% %   & \ \  \mathrlap{\{\mu_s, s\in\mathbf{T_t^+}\}, \{\psi_s, s\in\mathbf{T_{t+1}}\},   \text{   such that:} } \\ \\ \hline \\
%      0 &= \nabla_{u_s^i} \bigg[ l_s^{i} + f^\intercal \lambda_{s}^i - h_s^{i\intercal} \mu_s^i  -  g_s^{i^\intercal} \gamma_s^i    &\bigg]_{x_s^*,u_s^*}, \ \ &i\in\mathbf{N}, \ s \in \mathbf{T_t} \\
%      0 &= \nabla_{x_s} \bigg[ l_s^i - \lambda_{s-1}^i + f^\intercal \lambda_{s}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i \bigg]_{x_{s}^*,u_{s}^*} - K_s^{-i\intercal} \psi_s^i, &  \  &i\in\mathbf{N}, \ s\in\mathbf{T_{t+1}}, \\
%      0 &= \nabla_{u^{-i}_s} \bigg[ l_s^i + f^\intercal \lambda_{s}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i  + \psi_s^i &\bigg]_{x_s^*,u_s^*},   \  &i\in\mathbf{N}, \ s\in\mathbf{T_{t+1}}, \\
%      0 &= \nabla_{x_{T+1}} \bigg[ l_{T+1}^i - \lambda_{T}^i - h_{T+1}^{i^\intercal} \mu_{T+1}^i  -  g_{T+1}^{i\intercal} \gamma_{T+1}^i &\bigg]_{x_{T+1}^*},  \  &i\in\mathbf{N}, \\
%     0 &= x^*_{s+1} - f(x^*_s,u^*_s), &&s\in\mathbf{T_t}, \\
%     0 &= h_s^i(x_s^*,u_s^*), &&i\in\mathbf{N}, \ s\in\mathbf{T_t},\\
%     0 &\leq g_s^i(x_s^*,u_s^*) \perp \gamma_s^i \geq 0, &&i\in\mathbf{N}, \ s\in\mathbf{T_t}, \\
%     0 &= h_{T+1}^i(x_{T+1}^*), &&i\in\mathbf{N},\\
%     0 &\leq g_{T+1}^i(x_{T+1}^*) \perp \gamma_{T+1}^i \geq 0, &&i\in\mathbf{N}. \Bigg\}
%     \end{alignat}
% \end{subequations}
% Above, $K_t^{-i}$ is defined as the following. Let \begin{equation}
%     \mathbf{z^i_t} := (x^*_{t+1:T+1}, u^{i*}_t, u^*_{t+1:T}, \lambda^i_{t:T}, \mu^i_{t:T+1}, \gamma^i_{t:T+1}, \psi^i_{t+1:T})
% \end{equation} represent the set of all primal and dual decision variables associated with the optimization problem \cref{eq:gqn_problem_T,eq:gqn_problem_t} of player $i\in\mathbf{N}$. Then let $G^i_t(x^*_t, u^{*-i}_t, \mathbf{z^i_t}) = 0$ represent the first-order necessary conditions of problems \cref{eq:gqn_problem_T,eq:gqn_problem_t} for that player (i.e. the conditions appearing in \cref{eq:qfoncs} for a particular $i\in\mathbf{N}$), where for each $j\in\{1,...,b_s^i\}$, if $g_{s,j}^i(x_s,u_s) > 0$, the inequality $g_{s,j}^i(x_s^*,u_s^*) \geq 0$ is replaced with $\gamma_{s,j}^i = 0$, otherwise it is replaced with the condition $g_{s,j}^i(x_s^*,u_s^*) = 0$. In other words, inactive inequality constraints are ignored, and active constraints are treated as equality constraints. Then the matrices $K_t^i$ are then defined to be the implicit Jacobian matrices relating first-order perturbations in $x^*_t$ to perturbations in $u^{*i}_t$ along solutions satisfying \cref{eq:qfoncs}:

% \begin{equation}
%     \label{eq:qpolicy_grad}
%     \begin{aligned}
%      \mathbf{K^i_{x,t}} &:= -[\nabla_{\mathbf{z^i_t}} G_t(x_t^*,u^{-i*}_t, \mathbf{z_t^i})]^{\dagger} [\nabla_{x_t}G_t(x_t^*,u^{-i*}_t,\mathbf{z_t^i})], \\
%       \mathbf{K^i_{u^{-i},t}} &:= -[\nabla_{\mathbf{z^i_t}} G_t(x_t^*,u^{-i*}_t, \mathbf{z_t^i})]^\dagger  [\nabla_{u^{-i}_t}G_t(x_t^*,u^{-i*}_t,\mathbf{z_t^i})], \\
%     K_{x,t}^i &:= [\mathbf{K^i_{x,t}}]_{u^i_t}, \\ 
%     K_{u^{-i},t}^i &:= [\mathbf{K^i_{u^{-i},t}}]_{u^i_t} := [K_{u^{1},t}^i,...K_{u^{i-1},t}^i,K_{u^{i+1},t}^i,...,K_{u^{N},t}^i], \\
%     \begin{bmatrix}
%     K_t^1 \\ \vdots \\ K_t^N 
%     \end{bmatrix} &:= -
%     \begin{bmatrix}
%     I & -K_{u^{2},t}^1 & \hdots & -K_{u^N,t}^1 \\
%     -K_{u^1,t}^2 & I & \ddots & \vdots \\
%     \vdots & \ddots & \ddots & -K_{u^N,t}^{N-1} \\
%     -K_{u^1,t}^N & \hdots & -K_{u^{N-1},t}^N & I
%     \end{bmatrix}^{-1} 
%     \begin{bmatrix}  
%     K_{x,t}^1 \\ \vdots \\ K_{x,t}^N
%     \end{bmatrix}
%     \end{aligned}
% \end{equation} Above, the notation $[\mathbf{K^i_{x,t}}]_{u_t^i}$ indicates that if $u_t^i$ appears in the $j_1$ through $j_2$ indices of $\mathbf{z^i_t}$, then $K_{x,t}^i$ corresponds to the the $j_1$ through $j_2$ rows of the matrix $\mathbf{K^i_{x,t}}$. The notation $[\cdot]^\dagger$ is used to represent the Moore-Penrose inverse. The need for using this generalized inverse instead of the matrix inverse is discussed below.
% $K_t^{-i}$ is then defined as 
% \begin{equation}
%     K_t^{-i} := \begin{bmatrix} (K_t^1)^\intercal & \hdots & (K_t^{i-1})^\intercal & (K_t^{i+1})^\intercal & \hdots & (K_t^N)^\intercal
%     \end{bmatrix}^\intercal.
% \end{equation}
% \end{theorem}

% \begin{proof}
% The proof of \cref{thm:qfoncs} can be made by induction. For stage $t=T$, the conditions \cref{eq:qfoncs} are exactly those in \cref{eq:foncs}, since the set $\mathbf{T_{T+1}} = \emptyset$. Assume now that for some stage $t+1$, the first-order necessary conditions for \cref{eq:gqn_problem_T} or \cref{eq:gqn_problem_t} are given by the conditions in \cref{eq:qfoncs}, as holds for the base case $t+1=T$. The conditions in \cref{eq:qfoncs} form a mixed-complementarity system, and all the functions appearing in those conditions are continuously differentiable. Therefore, in some neighborhood of $u_t, x_t$ satisfying \cref{eq:generalized_constraints}, by Robinson's Implicit Function Theorem\fnote{check/cite}, there exists a neighborhood around $x_t$ such that there exists a Lipshitz-continuous function implicitly defined by the conditions \cref{eq:qfoncs} mapping $x_t$ to $u_t$. Furthermore, under the assumption of strict-complementarity, the implicit function is differentiable at the point $x_t$, and it's gradient is given by 
% \begin{equation}
%     K_t := \begin{bmatrix} (K_t^1)^\intercal & \hdots & (K_t^N)^\intercal \end{bmatrix}^\intercal,
% \end{equation}
% where $K_t^i$, $i\in\mathbf{N}$ are defined as above. $K_t$ is guaranteed to exist, even in the case that the Jacobian matrix $\nabla_{\mathbf{z_t}} G_t(x_t^*,\mathbf{z_t})$ is singular, since 

% By concatenating the KKT conditions associated with the problems \cref{eq:gqn_problem_t}, the following conditions are formed: 

% \begin{subequations}
%     \label{eq:qfoncs_redundant}
%     \begin{alignat}{3}
% %   & \mathrlap{\Gamma_t(x^*_t) := \Bigg\{ u^*_t \ : \ \exists x^*_{t+1:T+1}, u^*_{t+1:T}, \lambda_{t:T}, \mu_{t:T+1}, \gamma_{t:T+1}, \psi_{t+1:T}:} \\
% %   & \ \ \ \Updownarrow \\
% %   &\mathrlap{\exists \{x_{s+1}, s\in\mathbf{T_t}\}, \{u_s, s\in\mathbf{T_{t+1}}\}, \{\lambda_s, s\in\mathbf{T_t^+}\},} \\
% %   & \ \  \mathrlap{\{\mu_s, s\in\mathbf{T_t^+}\}, \{\psi_s, s\in\mathbf{T_{t+1}}\},   \text{   such that:} } \\ \\ \hline \\
%      0 &= \nabla_{u_t^i} \bigg[ l_t^{i} + f^\intercal \lambda_{t}^i - h_t^{i\intercal} \mu_t^i  -  g_t^{i^\intercal} \gamma_t^i  &\bigg]_{x_t^*,u_t^*}, \ \ &i\in\mathbf{N} \\
%     0 &= \nabla_{u_s^i} \bigg[ l_s^{i} + f^\intercal \lambda_{s}^i - h_s^{i\intercal} \mu_s^i  -  g_s^{i^\intercal} \gamma_s^i + \psi_s^{i,i} &\bigg]_{x_s^*,u_s^*}, \ \ &i\in\mathbf{N}, \ s \in \mathbf{T_{t+1}} \label{eq:qfoncs_r1} \\
%      0 &= \nabla_{x_s} \bigg[ l_s^i - \lambda_{s-1}^i + f^\intercal \lambda_{s}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i \bigg]_{x_{s}^*,u_{s}^*} - K_s^{\intercal} \psi_s^i, &  \  &i\in\mathbf{N}, \ s\in\mathbf{T_{t+1}}, \label{eq:qfoncs_r2}\\
%      0 &= \nabla_{u^{-i}_s} \bigg[ l_s^i + f^\intercal \lambda_{s}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i  + \psi_s^{i,-i} &\bigg]_{x_s^*,u_s^*},   \  &i\in\mathbf{N}, \ s\in\mathbf{T_{t+1}}, \label{eq:qfoncs_r3} \\
%      0 &= \nabla_{x_{T+1}} \bigg[ l_{T+1}^i - \lambda_{T}^i - h_{T+1}^{i^\intercal} \mu_{T+1}^i  -  g_{T+1}^{i\intercal} \gamma_{T+1}^i &\bigg]_{x_{T+1}^*},  \  &i\in\mathbf{N}, \label{eq:qfoncs_r4} \\
%     0 &= x^*_{s+1} - f(x^*_s,u^*_s), &&s\in\mathbf{T_t}, \label{eq:qfoncs_r5}\\
%     0 &= h_s^i(x_s^*,u_s^*), &&i\in\mathbf{N}, \ s\in\mathbf{T_t},\label{eq:qfoncs_r6}\\
%     0 &\leq g_s^i(x_s^*,u_s^*) \perp \gamma_s^i \geq 0, &&i\in\mathbf{N}, \ s\in\mathbf{T_t}, \label{eq:qfoncs_r7}\\
%     0 &= h_{T+1}^i(x_{T+1}^*), &&i\in\mathbf{N},\label{eq:qfoncs_r8}\\
%     0 &\leq g_{T+1}^i(x_{T+1}^*) \perp \gamma_{T+1}^i \geq 0, &&i\in\mathbf{N}, \label{eq:qfoncs_r9}\\
%     0 & \in (u_s^{i*},u_s^{-i*}) -\Gamma_s(x_s^*), &&s\in\mathbf{T_{t+1}}. \label{eq:redundant_remove} \Bigg\}
%     \end{alignat}
% \end{subequations}
% Above, the multipliers $\psi_s^i := (\psi_s^{i,i},\psi_s^{i,-i})$ are the Lagrange multipliers of player $i$ associated with the shared constraint \cref{eq:redundant_remove} at stage $s$. Notice that the set of conditions \cref{eq:qfoncs_r1}, \cref{eq:qfoncs_r2,eq:qfoncs_r3} excluding $s=t+1$,   \cref{eq:qfoncs_r5,eq:qfoncs_r6,eq:qfoncs_r6} excluding $s=t$, and \cref{eq:qfoncs_r4,eq:qfoncs_r8,eq:qfoncs_r9} together constitute the conditions \cref{eq:qfoncs} evaluated at $t+1$, with the exception being the presence of the term $\psi_s^{i,i}$ appearing in \cref{eq:qfoncs_r1}. However, the conditions \cref{eq:qfoncs} in their original form are also included in \cref{eq:qfoncs_redundant}, in the form of \cref{eq:redundant_remove}. This implies that $\psi_s^{i,i}$ must be $0$ for \cref{eq:qfoncs_redundant} to be satisfied, and can therefore be ignored. This then implies that the conditions \cref{eq:redundant_remove} are strictly redundant as well, and can also be removed. Eliminating these conditions leaves exactly the conditions \cref{eq:qfoncs} for stage $t$, as desired. Therefore, since \cref{eq:qfoncs} represent the first-order necessary conditions for \cref{eq:gqn_problem_T}, and must also represent the first-order necessary conditions for \cref{eq:gqn_problem_t} at stage $t$ if they do at stage $t+1$, the conditions \cref{eq:qfoncs} indeed must represent the first-order necessary conditions for the problems \cref{eq:gqn_problem_T,eq:gqn_problem_t} at all stages $t\in\mathbf{T}$. \end{proof}

% \begin{subequations}
%     \label{eq:qfoncs_redundant2}
%     \begin{alignat}{3}
%      0 &= \nabla_{u_t^i} \bigg[ l_t^{i} + f^\intercal \lambda_{t}^i - h_t^{i\intercal} \mu_t^i  -  g_t^{i^\intercal} \gamma_t^i  &\bigg]_{x_t^*,u_t^*}, \ \ &i\in\mathbf{N} \\
%      0 &= \nabla_{x_{t+1}} \bigg[ l_{t+1}^i - \lambda_{t}^i + f^\intercal \lambda_{t+1}^i - h_{t+1}^{i^\intercal} \mu_{t+1}^i  -  g_{t+1}^{i\intercal} \gamma_{t+1}^i \bigg]_{x_{t+1}^*,u_{t+1}^*} - K_{t+1}^{\intercal} \psi_{t+1}^i, &  \  &i\in\mathbf{N}, \\
%          0 &= \nabla_{u_{t+1}^i} \bigg[ l_{t+1}^{i} + f^\intercal \lambda_{t+1}^i - h_{t+1}^{i\intercal} \mu_{t+1}^i  -  g_{t+1}^{i^\intercal} \gamma_{t+1}^i + \psi_{t+1}^{i,i} &\bigg]_{x_{t+1}^*,u_{t+1}^*}, \ \ &i\in\mathbf{N}\\
%     0 &= \nabla_{u_s^i} \bigg[ l_s^{i} + f^\intercal \lambda_{s}^i - h_s^{i\intercal} \mu_s^i  -  g_s^{i^\intercal} \gamma_s^i + \psi_s^{i,i} &\bigg]_{x_s^*,u_s^*}, \ \ &i\in\mathbf{N}, \ s \in \mathbf{T_{t+2}} \\
%      0 &= \nabla_{x_s} \bigg[ l_s^i - \lambda_{s-1}^i + f^\intercal \lambda_{s}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i \bigg]_{x_{s}^*,u_{s}^*} - K_s^{\intercal} \psi_s^i, &  \  &i\in\mathbf{N}, \ s\in\mathbf{T_{t+2}}, \\
%      0 &= \nabla_{u^{-i}_s} \bigg[ l_s^i + f^\intercal \lambda_{s}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i  + \psi_s^{i,-i} &\bigg]_{x_s^*,u_s^*},   \  &i\in\mathbf{N}, \ s\in\mathbf{T_{t+1}}, \\
%      0 &= \nabla_{x_{T+1}} \bigg[ l_{T+1}^i - \lambda_{T}^i - h_{T+1}^{i^\intercal} \mu_{T+1}^i  -  g_{T+1}^{i\intercal} \gamma_{T+1}^i &\bigg]_{x_{T+1}^*},  \  &i\in\mathbf{N}, \\
%     0 &= x^*_{s+1} - f(x^*_s,u^*_s), &&s\in\mathbf{T_t}, \\
%     0 &= h_s^i(x_s^*,u_s^*), &&i\in\mathbf{N}, \ s\in\mathbf{T_t},\\
%     0 &\leq g_s^i(x_s^*,u_s^*) \perp \gamma_s^i \geq 0, &&i\in\mathbf{N}, \ s\in\mathbf{T_t}, \\
%     0 &= h_{T+1}^i(x_{T+1}^*), &&i\in\mathbf{N},\\
%     0 &\leq g_{T+1}^i(x_{T+1}^*) \perp \gamma_{T+1}^i \geq 0, &&i\in\mathbf{N}, \\
%     0 & \in (u_s^{i*},u_s^{-i*}) -\Gamma_s(x_s^*), &&s\in\mathbf{T_t}. \Bigg\}
%     \end{alignat}
% \end{subequations}


% The constraints \cref{eq:generalized_constraints} appearing in \cref{eq:gqn_problem_t} can be equivalently expressed replacing them with the conditions in \cref{eq:qfoncs} (and adding the corresponding dual multipliers to the optimization \cref{eq:gqn_problem_t}), which are assumed equivalent by our inductive hypothesis. However, it can be seen immediately that many of the resultant constraints are redundant, as for example the dynamic and non-dynamic constraints appearing in \cref{eq:qfoncs} already appear in \cref{eq:gqn_problem_t}. 


% The conditions appearing in \cref{eq:qfoncs} are formed by expressing the concatenated first-order necessary conditions of \cref{eq:gqn_problem_t}, with the omission of the constraints \cref{eq:generalized_constraints}. The term $\nabla{x_s} \Gamma_s(x_s)$ still appears however. This omission is due to redundancy, as shown in the following. Let the set of variables appearing in \cref{eq:qfoncs} other than $x^*_t$ be denoted by $\mathbf{z^*_t}$. Then the entire set of conditions appearing in \cref{eq:qfoncs} can be compactly expressed as the mixed complementarity system, 
% \begin{equation}
%     \label{eq:mcp_compact}
%     0 \leq \mathbf{M_t}_j(\mathbf{z^*_t},x_t^*) \perp \mathbf{z^*_t}_j \geq \mathbf{b_t}_j,
% \end{equation}
% where $\mathbf{M_t(z^*_t},x_t^*)$ denotes the concatenation of all terms appearing in the right-hand side of \cref{eq:qfoncs}, and $\mathbf{b_t}$ is a vector of lower-bounds, with $\mathbf{b_t}_j = 0$ if $\mathbf{M_t}_j(\mathbf{z^*_t},x_t^*)$ corresponds to an inequality in \cref{eq:qfoncs}, else $\mathbf{b_t}_j = -\infty$. Here $j$ indexes individual elements of these vectors, of which we denote the total size by $d_t$, i.e. $j\in\mathbf{d_t}:={1,...,d_t\}$. Note that the existence of variables satisfying the set of conditions in \cref{eq:qfoncs}, and therefore \cref{eq:mcp_compact}, are equivalent to the constraint $u_t \in \Gamma_t(x_t)$. 

% From the form introduced, it can be made explicit that the constraint $u_{t+1} \in \Gamma_{t+1}(x_{t+1})$ is included in \cref{eq:qfoncs}. We re-write these conditions as the following:

% \begin{subequations}
%     \label{eq:qfoncs_nested}
%     \begin{alignat}{3}
%      0 &= \nabla_{u_t^i} \bigg[ l_t^{i} + f^\intercal \lambda_{t}^i - h_t^{i\intercal} \mu_t^i  -  g_t^{i^\intercal} \gamma_t^i    &\bigg]_{x_t^*,u_t^*}, \ &i\in\mathbf{N}, \\
%      0 &= \nabla_{x_{t+1}} \bigg[ l_{t+1}^i - \lambda_{t}^i + f^\intercal \lambda_{t+1}^i - h_{t+1}^{i^\intercal} \mu_{t+1}^i  -  g_{t+1}^{i\intercal} \gamma_{t+1}^i  - \Gamma_{t+1}^\intercal \psi_{t+1}^i &\bigg]_{x_{t+1}^*,u_{t+1}^*},   \  &i\in\mathbf{N}, \label{eq:qfnested_xt} \\
%      0 &= \nabla_{u^{-i}_{t+1}} \bigg[ l_{t+1}^i + f^\intercal \lambda_{t+2}^i - h_{t+1}^{i^\intercal} \mu_{t+1}^i  -  g_{t+1}^{i\intercal} \gamma_{t+1}^i  + \psi_{t+1}^i &\bigg]_{x_{t+1}^*,u_{t+1}^*},   \  &i\in\mathbf{N}, \label{eq:qfnested_uot} \\
%     0 &= x^*_{t+1} - f(x^*_t,u^*_t), \\
%     0 &= h_t^i(x_t^*,u_t^*), &&i\in\mathbf{N},\\
%     0 &\leq g_t^i(x_t^*,u_t^*) \perp \gamma_t^i \geq 0, &&i\in\mathbf{N}, \\
%     0 &\leq \mathbf{M_{t+1}}_j(\mathbf{z^*_{t+1}},x_{t+1}^*) \perp \mathbf{z^*_{t+1}}_j \geq \mathbf{b_{t+1}}_j,  &&j\in\mathbf{d_{t+1}} \label{eq:mcp_form}
%     \end{alignat}
% \end{subequations}
% Here the conditions in \cref{eq:mcp_form} are equivalent to $u_{t+1}\in\Gamma_{t+1}(x_{t+1})$. By a recursive argument, the same holds for all conditions  $\tilde{u_{s}} \in \Gamma_{s}(x_{s})$, $s\in\mathbf{T_{t+1}}$. Therefore, those constraints need not be included in \cref{eq:qfoncs} to represent the first-order necessary conditions of problems \cref{eq:gqn_problem_t} evaluated at stage $t$. It is important to note that the inclusion of these constraints are only redundant when expressing the first-order necessary conditions of the problems \cref{eq:gqn_problem_t} for all players $i\in\mathbf{N}$ simultaneously. 


% The first-order necessary conditions associated with a GQFNE

% \dfknote{It would be good if we explained the diff}
% Let $z_t := (\lambda_t, \mu_t, \gamma_t, \psi_t, x_{t+1},u_{t+1}, \lambda_{t+1},...,x_{T+1},\lambda_{T+1},\mu_{T+1},\gamma_{T+1})$. Then let $\mathbf{q_t}(u_t,z_t;x_t)$ denote the concatenation of the right-hand-side of all conditions listed in \cref{eq:qfoncs}. We can then equivalently express these conditions in abbreviated form as the following Variational Inequality:
% \begin{equation}
%     \label{eq:VI}
%     VI_t(\mathbf{q}, [\mathbf{a_t},\ \mathbf{\infty}])
% \end{equation}
% Above, $\mathbf{a}$ has dimension equal to that of $\mathbf{q_t}$. For every element of $\mathbf{a_t}$, denoted $\mathbf{a_t}_k$, if $\mathbf{q_t}_k$ corresponds to a complementarity condition, $\mathbf{a_t}_k = -\infty$. Otherwise, $\mathbf{a_t}_k = 0$. 

% \begin{theorem}
% \label{thm:vi_implicit}
% Assume the policies $\hat{\pi}_s(\cdot)$ are known for $s > t$. Let $x_t^*$ be such that there exist states $x_s^*$, $s\in\mathbf{T_{t+1}^+}$, controls $u_s^*$, $s\in\mathbf{T_t}$, and multipliers satisfying \cref{eq:qfoncs}, and that strict complementarity holds. Then the policy $\hat{\pi}_t(x_t^*)$ and policy gradient $\nabla \hat{\pi}_t(x_t^*)$ are defined implicitly by \cref{eq:qfoncs}. 
% \end{theorem}

% \begin{definition}[Implicit Quasi-Policy Gradients]
%     We refer to the policies $\hat{\pi}_t(x_t)$ as quasi-policies, which, along with their corresponding gradients, $\nabla_{x_t}\hat{\pi}_t(x_t)$, are defined implicitly in terms of the conditions \cref{eq:qfoncs}, via \cref{thm:vi_implicit} \\\fnote{Need to be careful with active set, etc., also not really a function.}
% \end{definition}

% \begin{definition}[GFQNE]
%     A Generalized Feedback Quasi-Nash Equilibrium is any set of $\{u^{i*}_t; t\in\mathbf{T}, i\in\mathbf{N}\}$, $\{x^*_t; t\in\mathbf{T^+}\}$, $\{\lambda_t^i\in\mathbb{R}^n; \ t\in\mathbf{T}, \ i\in\mathbf{N}\}$, $\{\mu_t^i\in\mathbb{R}^{k^i_t}; \ t\in\mathbf{T^+}, \ i\in\mathbf{N}\}$, $\{\gamma_t^i\in\mathbb{R}^{j^i_t}; \ t\in\mathbf{T^+}, \ i\in\mathbf{N}\}$, and $\{\psi_t^i\in\mathbb{R}^{m^{-i}};\ t\in\mathbf{T_{2}}, \ i\in\mathbf{N}\}$ which together satisfy the conditions \cref{eq:qfoncs} evaluated at $t=1$ and $x_1^*=\xinit$. 
% \end{definition}

% While the trajectories associated with a GFQNE may not satisfy any second-order conditions on the sub-game policies appearing in the game, these approximations are far more amenable to computing numerical solutions. The conditions \cref{eq:qfoncs} only require the evaluation of the sub-game policy gradients, $\nabla_{x_s}\Gamma_s(x_s)$, and not evaluation of the policies themselves. Note that an explicit representation of these policy gradients is not generally available, however they are implicitly defined and can be evaluated, as stated in the following. 

% \begin{theorem}
% Consider the first-order necessary conditions associated with the problems \cref{eq:gqn_problem_t} evaluated at stage $t=T$. These conditions are as stated in \cref{eq:qfoncs_nested} when omitting \cref{eq:qfnested_xt,eq:qfnested_uot,eq:mcp_form}. We express these conditions as 
% \begin{equation}
%     \label{eq:mcp_compact_T}
%     0 \leq \mathbf{M_T}_j(\mathbf{z^*_T},x_T^*) \perp \mathbf{z^*_T}_j \geq \mathbf{b_T}_j, \ \ j\in\mathbf{d_T}
% \end{equation} as was done in \cref{eq:mcp_compact}. For any such $\mathbf{z_T^*},x_T^*$ satisfying conditions \cref{eq:mcp_compact_T}, assume that strict complementarity holds, meaning $\mathbf{M_T}_j(\mathbf{z^*_T},x_T^*)=0$ iff $\mathbf{z^*_T} > \mathbf{b_T}_j$.
% \end{theorem}

% \cref{thm:qfoncs} states that when searching for a trajectory satisfying the first-order necessary conditions of a GFQNE, the explicit form of the GFQNE policies does not need to be known---only the \emph{policy gradients} \cref{eq:qpolicy_grad} evaluated about the trajectory need be known. This fact is particularly important for computational purposes, as the policies \cref{eq:gqn_problem_T,eq:gqn_problem_t} are in general highly nonlinear and impossible to represent explicitly. While an explicit representation of the policies is no longer needed, there still remain significant challenges to evaluating the policy gradients \cref{eq:qpolicy_grad} which must be addressed in order to develop numerical methods capable of finding solutions to \cref{eq:qfoncs}. 

% By \cref{thm:foncs}, in order to evaluate the gradients of the quasi-policies appearing in \cref{eq:qfoncs} at some stage $t$, $\nabla_{x_t}\hat{\pi}_t(x_t)$, higher order derivatives of all policies $\hat{\pi}_{s}(x_s)$, $s\in\mathbf{T_{t+1}}$ must be evaluated. At the extreme, evaluating the conditions \cref{eq:qfoncs} at $s=1$ involves taking $(T-1)$-order derivatives of the expressions appearing in \cref{eq:qfoncs} evaluated at $s=T$. \fnote{check this is correct, might be off by $\pm 1$}

% The evaluation of these higher-order derivatives can pose significant difficulties for numerical methods. We therefore introduce yet another approximation to the conditions \cref{eq:qfoncs} which is amenable to numerical methods in the general case. This approximation will be defined in terms of yet another set of policies, $\bar{\pi}_t(x_t)$. The principle idea behind this approximation is to ignore non-first-order derivatives of the policies $\bar{\pi}_s(x_s)$ in the definition of the policy $\bar{\pi}_t(x_t)$, with $s>t$. To this end, we make use the following definition.

% \begin{definition}[Truncated Gradient]
% Consider a function $p : \mathbb{R}^{d^1} \to \mathbb{R}^{d^2}$. Then the $k$th-order truncated gradient of $p$ evaluated at $y\in\mathbb{R}^{d^1}$, denoted $\nabla^{(k)}p(y)$, is defined as the following:
% \begin{equation}
%     \mathcal{D}^{j-1}\nabla^{(k)}p(y) = \left\{ \begin{array}{cl} \mathcal{D}^j p(y), &j \leq k \\ 0, &\text{else} \end{array}
%                                      \right\},
% \end{equation}
% where $\mathcal{D}^i$ is the $i$th-order derivative operator (e.g. $\mathcal{D}^1p := \nabla p$, and $\mathcal{D}^0p:=p$). \dfknote{This defn makes sense only when I parse it a bunch of times. I think my own confusion is in the use of $\nabla$ to represent the function itself (with truncated derivatives) and not the derivative itself (as it normally would, and as this last parenthetical is implying). My suggestion would be to use a different symbol, maybe one option would be to use $\mathcal{T}$ (as in, \emph{truncated} gradient).}
% \end{definition}

% The modified version of the conditions \cref{eq:qfoncs} are the following.

% \begin{equation}
%     \label{eq:tfoncs}
%     \begin{alignedat}{3}
%      0 &= \nabla_{u_s^i} \bigg[ l_s^{i} + f^\intercal \lambda_{s}^i - h_s^{i\intercal} \mu_s^i  -  g_s^{i^\intercal} \gamma_s^i    &\bigg]_{x_s^*,u_s^*}, \ \ &i\in\mathbf{N}, \ s \in \mathbf{T_t} \\
%      0 &= \nabla_{x_s} \bigg[ l_s^i - \lambda_{s-1}^i + f^\intercal \lambda_{s}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i \bigg]_{x_s^*,u_s^*}  + &\nabla^{(1)}\bar{\pi}_s^{-i*\intercal}\psi_s^i,  \ \ &i\in\mathbf{N}, \ s\in\mathbf{T_{t+1}}, \\
%      0 &= \nabla_{u^{-i}_s} \bigg[ l_s^i + f^\intercal \lambda_{s+1}^i - h_s^{i^\intercal} \mu_s^i  -  g_s^{i\intercal} \gamma_s^i  - \psi_s^i &\bigg]_{x_s^*,u_s^*},   \ \ &i\in\mathbf{N}, \ s\in\mathbf{T_{t+1}}, \\
%      0 &= \nabla_{x_{T+1}} \bigg[ l_{T+1}^i - \lambda_{T+1}^i - h_{T+1}^{i^\intercal} \mu_{T+1}^i  -  g_{T+1}^{i\intercal} \gamma_{T+1}^i &\bigg]_{x_{T+1}^*},  \ \ &i\in\mathbf{N}, \\
%     0 &= x^*_{s+1} - f(x^*_s,u^*_s), &&s\in\mathbf{T_t}, \\
%     0 &= h_s^i(x_s^*,u_s^*), &&i\in\mathbf{N}, \ s\in\mathbf{T_t},\\
%     0 &\leq g_s^i(x_s^*,u_s^*) \perp \gamma_s^i \geq 0, &&i\in\mathbf{N}, \ s\in\mathbf{T_t}, \\
%     0 &= h_{T+1}^i(x_{T+1}^*), &&i\in\mathbf{N},\\
%     0 &\leq g_{T+1}^i(x_{T+1}^*) \perp \gamma_{T+1}^i \geq 0, &&i\in\mathbf{N}.
%     \end{alignedat}
% \end{equation}

% The term $\nabla^{(1)}\bar{\pi}_s^*$ is the first-order truncated gradient of the policy $\bar{\pi}_s(\cdot)$, evaluated at $x_s^*$. \dfknote{I think we need to be a little more precise here, using the notation from the defn above.}

% \begin{definition}[Implicit Truncated Policies]
%     We refer to the policies $\bar{\pi_t}(x_t)$ as truncated feedback policies, which, along with their corresponding gradients, $\nabla_{x_t}\bar{\pi}_t(x_t)$, are defined implicitly in terms of the conditions \cref{eq:tfoncs}, via \cref{thm:vi_implicit} \\\fnote{Need to be really careful. .}
% \end{definition}


% \begin{definition}[GTFQNE]
% A Generalized Truncated Feedback Quasi-Nash\\ Equilibrium is any set of $\{u^{i*}_t; t\in\mathbf{T}, i\in\mathbf{N}\}$, $\{x^*_t; t\in\mathbf{T^+}\}$, $\{\lambda_t^i\in\mathbb{R}^n; \ t\in\mathbf{T}, \ i\in\mathbf{N}\}$, $\{\mu_t^i\in\mathbb{R}^{k^i_t}; \ t\in\mathbf{T^+}, \ i\in\mathbf{N}\}$, $\{\gamma_t^i\in\mathbb{R}^{j^i_t}; \ t\in\mathbf{T^+}, \ i\in\mathbf{N}\}$, and $\{\psi_t^i\in\mathbb{R}^{m^{-i}};\ t\in\mathbf{T_{2}}, \ i\in\mathbf{N}\}$ which together satisfy the conditions \cref{eq:tfoncs} evaluated at $t=1$ and $x_1^*=x_1$. 
% \end{definition}

% Borrowing ideas from the method for constrained Algebraic Riccati recursion presented in \cite{laine2019efficient}, we extend the formulation for LQ Feedback Nash presented in \cite{basar1998dynamic} to the constrained case considered here. 

% Taking a dynamic programming perspective, assume that at each stage $t$, the value function for player $i$, defined in  \cref{eq:value_function_terminal,eq:value_functions}, is given by
% \begin{equation}
%     \label{eq:extended_quadratic_value}
%     V_t^i(x_t) :=  \left\{ \begin{array}{cc}
%          \frac{1}{2} x_t^\intercal P_t^i x_t + x_t^\intercal p_t^i, & D_t^i x_t + d^i_t = 0  \\
%          \infty & \text{else,}
%     \end{array}\right.
% \end{equation}

% for appropriate coefficients $P_t^i$, $p_t^i$, $D_t^i$, and $d_t^i$. Let the dimension of the linear constraint appearing in \cref{eq:extended_quadratic_value} be given by $e_t^i$, i.e. $d_t^i \in \mathbb{R}^{e_t^i}$.



% % associated with a quadratic \emph{cost-to-go}, defined by the form 
% % \begin{equation}
% %     \label{eq:cost_to_go}
% %   \frac{1}{2} x_t^\intercal P_t^i x_t + x_t^\intercal p_t^i.
% % \end{equation}
% % Furthermore, assume that each player is associated with a linear \emph{constraint-to-go} at stage $t$, defined by the form 
% % \begin{equation}
% %     \label{eq:constraint_to_go}
% %     D_t^i x_t + d^i_t = 0,
% % \end{equation}
% % where the dimension of this constraint is given by $e_t^i$, i.e. $d_t^i \in \mathbb{R}^{e_t^i}$. Together, the cost-to-go and constraint-to-go for each player identifies the cost of the remainder of the trajectory starting from state $x_t$ at stage $t$, assuming all players adhere to the policies $\hat{\pi}_s$, for $s>t$. Specifically, we have that the value function for player $i$, defined in  \cref{eq:value_function_terminal,eq:value_functions}, is given by
% % \begin{equation}
% %     \label{eq:extended_quadratic_value}
% %     V_t^i(x_t) :=  \left\{ \begin{array}{cc}
% %          \frac{1}{2} x_t^\intercal P_t^i x_t + x_t^\intercal p_t^i, & D_t^i x_t + d^i_t = 0  \\
% %          \infty & \text{else}
% %     \end{array}\right.
% % \end{equation}

% We prove that the form of this value function is valid for all $t\in\mathbf{T^+}$, which we show by an inductive argument. Note that for stage $t=T+1$, this assumption indeed holds, with the relationships  $P_{T+1}^i=Q_{T+1}^i$,  $p_{T+1}^i=q_{T+1}^i$,  $D_{T+1}^i=H_{X_{T+1}}^i$, and $d_{T+1}^i=h_{T+1}^i$. 

% % Now, assuming the cost-to-go and constraint-to-go are defined as above for stage $t+1$, we show how they can be derived for the preceding stage $t$, and that the policies $\hat{\pi}_t(x_t)$ are generated as a byproduct. 

% % Given the inductive hypothesis regarding the cost- and constraint-to-go forms, we first equivalently express \cref{eq:gn_problem_t,eq:gn_problem_T} in compact form:

% Assuming the form of the value functions at stage $t$ are given by \cref{eq:extended_quadratic_value}, the control-value functions are defined precisely as in \cref{eq:q_functions}, using the form of cost-functional and linear equality constraints given in \cref{eq:quadratic_cost_functional,eq:linear_eq_constraints}. This form can be represented as the following:

% % Define the policies 

% % \begin{theorem} 
% % For the dynamic game defined by \cref{eq:linear_eq_constraints,eq:quadratic_cost_functional,eq:linear_dynamics}, the policies $\pi_t(x_t)$ defined as 
% % \end{theorem}




% % \begin{equation}
% %     \label{eq:control-value-func-lq}
% %     Z_t^i(x_t,u_t^1,...,u_t^N) :=  \left\{\begin{array}{@{}ll@{}}
% %          \frac{1}{2}\Bigg( \begin{bmatrix} x_t\\u_t\end{bmatrix}^\intercal \begin{bmatrix} Q_t^i & S_t^{i\intercal} \\ S_t^i & R_t^i\end{bmatrix} \begin{bmatrix} x_t\\u_t\end{bmatrix} + 2\begin{bmatrix} x_t\\u_t\end{bmatrix}^\intercal \begin{bmatrix} q_t^i \\ r_t^i \end{bmatrix} \Bigg) \ + \\
% %     \frac{1}{2} \bigg(f(x_t,u_t)^\intercal \Big( P_{t+1}^i f(x_t,u_t) + 2p_{t+1}^i\Big)\bigg), & \multirow{2}{*}{$H^i_{x_t}x_t + H_{u_t}^iu_t + h_t^i=0$,} \\
% %     \\
% %         \infty, & \text{else}
% %         \end{array}\right. 

% % \underset{u_t^i }{\text{arg} \ } \underset{\substack{u_t,\\
% %     x_{t+1}}}{\text{min}}\ 
% % \end{equation}

% \begin{equation}
% \label{eq:prob_compact}
% \begin{alignedat}{3}
%     Z_t^i(x_t,u_t) &= 
%       \frac{1}{2}\bigg( \begin{bmatrix} x_t\\u_t\end{bmatrix}^\intercal \begin{bmatrix} Q_t^i & S_t^{i\intercal} \\ S_t^i & R_t^i\end{bmatrix} \begin{bmatrix} x_t\\u_t\end{bmatrix} + 2\begin{bmatrix} x_t\\u_t\end{bmatrix}^\intercal \begin{bmatrix} q_t^i \\ r_t^i \end{bmatrix} \Bigg) \ + \\
%     & \hspace{1.cm} \ \ \frac{1}{2} \bigg(f(x_t,u_t)^\intercal \big( P_{t+1}^i f(x_t,u_t) + 2 p_{t+1}^i\big)\bigg) \ + \\
%     & \hspace{1.cm} \ \ \mathcal{I}_{\infty}(H_{x_t}^i x_t + H_{u_t}^i u_t + h_t^i) + \mathcal{I}_{\infty}(D_{t+1}^i f(x_t,u_t) + d_{t+1}^i),
% \end{alignedat}
% \end{equation}
% Here we leverage the shorthand 
% \begin{equation}
%     \mathcal{I}_\infty(y) := \begin{cases} 0 & y=0\\ \infty & \text{else.}\end{cases}
% \end{equation}

% From this definition, we can propose candidate policies, $\pi^i_t(x_t)$, which will define a GFNE for this problem if one exists. 
% % \dfknote{Isn't $u^i_t$ duplicated in the arg min? also, i don't follow why the $u^{-i}$ term is there.} \fnote{Yeah so this is the notation I am trying out which indicates that we are minimizing over multiple variables, but only returning a subset of them. The reason we need $u^{-i}$ is to define that this is an equilibrium problem, and that parameters appearing in this problem ($u_t^{-i}$) are results of the optimization of other players.} 

% Expressing the first-order necessary conditions for the problem $\min_{u_t^i} Z_t^i(x_t,u_t)$, we have for each $i\in\mathbf{N}$,

% \begin{equation}
%     \label{eq:private_kkt}
%     \begin{vmatrix} R_t^{i,i,i} & & B_t^{i,\intercal} & -H_{u_t^i}^{i\intercal} \\
%     & P_{t+1}^i & -I & & -D_{t+1}^{i\intercal} \\
%     -B_t^i & I \\
%     H_{u_t^i}^i \\
%     & D_{t+1}^i
%     \end{vmatrix}\begin{bmatrix}u_t^i \\ x_{t+1} \\ \lambda_t^i \\ \mu_t^i \\ \mu_{t+1}^i \end{bmatrix} + \begin{bmatrix} 
%     R_t^{i,-i} \\ 0 \\ B_t^{-i} \\ H_{u^{-i}_t}^i \\ 0 
%     \end{bmatrix} u_t^{-i} = \begin{bmatrix} -S_t^{i,i}x_t-r_t^i \\  -p_{t+1}^i \\ -A_tx_t - c_t \\ -H_{x_t}^ix_t - h_t^i \\ -d_{t+1}^i
%     \end{bmatrix}.
% \end{equation}

% % \begin{equation}
% %     \label{eq:kkt_T}
% %     \begin{array}{|c|c|c|c|c|c}
% %      R_T^{1,1}u_T + B_t^{1\intercal}\lambda_{T}^i -H_{u_t^1}^{1\intercal}\mu_T^i & &  -r_T^1  & &  -S_T^{1,1} & \\
% %      \vdots && \vdots && \vdots \\
% %     R_T^{N,N}u_T + B_t^{N\intercal}\lambda_{T}^N -H_{u_t^N}^{N\intercal}\mu_T^N & & -r_T^N && -S_T^{N,N} & \\
% %     Q_{T+1}^1 x_{T+1} - \lambda_T^1 - H_{x_{T+1}}^{1\intercal}\mu_{T+1}^1 && -q_{T+1}^1 && 0 \\
% %     \vdots && \vdots && \vdots \\
% %     Q_{T+1}^N x_{T+1} - \lambda_T^N - H_{x_{T+1}}^{N\intercal}\mu_{T+1}^N && -q_{T+1}^N && 0 \\
% %     -B_T u_T & = & c_T & + & A_T & x_T\\
% %     H_{u_T}^1 u_T && -h_T^1 && -H_{x_T}^1 \\
% %     \vdots && \vdots && \vdots \\
% %     H_{u_T}^N u_T && -h_T^N && -H_{x_T}^N \\
% %     H_{x_{T+1}}^1 && -h_{T+1}^1 && 0 \\
% %     \vdots && \vdots && \vdots \\
% %     H_{x_{T+1}}^N && -h_{T+1}^N && 0 
% %     \end{array}.
% % \end{equation}

% The expression \cref{eq:private_kkt} can be expressed in compact form as 
% \begin{equation}
%     W^i_t \begin{bmatrix}\tilde{u}_t^i \\ x_{t+1} \\ \lambda_t^i \\ \mu_t^i \\ \mu_{t+1}^i \end{bmatrix} + W^{-i}_t \tilde{u}_t^{-i} = Y_t x_t + y_t
% \end{equation}
% Here $W^i_t$ is the matrix appearing in the left-hand side of \cref{eq:private_kkt}, $W_t^{-i}$ is the matrix of coefficients multiplying $\tilde{u}_t^{-i}$, and $Y_t x_t + y_t$ represent the right-hand-side. It can be seen that the matrix $W^i_t$ is square. If this matrix is full rank, the controls $\tilde{u}_t^i$ can be expressed in terms of $x_t$ and $\tilde{u}_t^{-i}$ simply as
% \begin{equation}
%     \label{eq:policy_in_terms_of_others}
%     \begin{aligned}
%     \tilde{u}_t^i &:= [(W_t^i)^{-1}]_{1:m^i}(-W_t^{-i}u_t^{-i} + Y_t x_t + y_t) \\
%     &:= \begin{bmatrix} \hat{W}_t^{i,1} & \hdots & \hat{W}_t^{i,i-1} & \hat{W}_t^{i,i+1} & \hdots & \hat{W}_t^{i,N} \end{bmatrix} \tilde{u}_t^{-i} + \hat{Y}_t^i x_t + \hat{y}_t^i
%     \end{aligned}
% \end{equation}
% \dfknote{the $-i$ superscript is really an inverse right? but that doesn't square with what follows. I'm lost. Oh wait I think you mean just $[W_t^i]_{1:m^i}]^{-1}$ on the left, and then below is what happens when you coalesce above for all $i$} where $[(W_t^i)^{-1}]_{1:m^i}$ denotes the first $m^i$ rows of $(W_t^i)^{-1}$, and $\hat{W}_t^{i,j}$, $\hat{Y}_t^i$, and $\hat{y}_t^i$ are introduced as shorthand. There exist controls $u_t^i$ jointly satisfying \cref{eq:private_kkt} if 
% \begin{equation}
%      \begin{bmatrix}  I & -\hat{W}_t^{1,2} & \hdots & -\hat{W}_t^{1,N} \\
%      -\hat{W}_t^{2,1} & I &  & \vdots \\
%      \vdots & &  \ddots  \\
%      -\hat{W}_{t}^{N,1} & \hdots & & I
%     \end{bmatrix} \tilde{u}_t = 
%     \begin{bmatrix} \hat{Y}_t^1 \\ \vdots \\ \hat{Y}_t^N \end{bmatrix} x_t + \begin{bmatrix} \hat{y}_t^i \\ \vdots \\ \hat{y}_t^N \end{bmatrix}
% \end{equation}



% % It can be verified \\ \fnote{(this will be super annoying to do notationally, but prove this)} that $W_T$ will be singular if any matrices of the form
% % \begin{equation}
% %     \begin{bmatrix} -B^i_T & I \\
% %     H_{u^i_T}^i & \\
% %     & H_{x_{T+1}}^i \end{bmatrix}
% % \end{equation} 
% % has rank $r > n+m^i$. 

% In general, the matrices $W_t^i$ may not be invertible. In particular, the matrix $W_t^i$ will be singular if and only if the matrix
% \begin{equation}
%     \begin{bmatrix} -B^i_t & I \\
%     H_{u^i_t}^i & \\
%     & D_{t+1}^i \end{bmatrix}
% \end{equation} 
% has rank $r > n+m^i$.\fnote{prove this via Schur complement or something.} 
% This is a common situation, and will occur if $e_{t+1}^i > m^i$ (the dimension of the constraint-to-go exceeds the control dimension). 

% In this setting, the conditions \cref{eq:private_kkt} do not have solutions for general values of $x_t$ and $u_t^{-i}$. However, if $x_t$ and $\tilde{u}_t^{-i}$ are such that a solution exists, it is given by $\hat{\pi}_t^i$, defined such that if $x_t$ and $u_t^{-i}$ satisfy
% \begin{equation}
%     \label{eq:player_i_feasible}
%     -W^{-i}_t \tilde{u}_t^{-i} + Y_t x_t + y_t \in\mathcal{C}(W^i_t),
% \end{equation} 
% where $\mathcal{C}(W^i_t)$ denotes the column-space of $W^i_t$, then there exist $\lambda_t^i$, $\mu^i_t$, $\mu^i_{t+1}$ such that
% \begin{equation}
%     \label{eq:player_i_g_inverse}
%      W^i_t \begin{bmatrix}\hat{\pi}^i_t(x_t) \\ x_{t+1} \\ \lambda_t^i \\ \mu_t^i \\ \mu_{t+1}^i \end{bmatrix} + W^{-i}_t \tilde{u}_t^{-i} = Y_t x_t + y_t.
% \end{equation} 
% We can therefore replace the term $(W_t^i)^{-1}$ appearing in \cref{eq:policy_in_terms_of_others} with $(W_t^i)^{g}$, where $(W_t^i)^g$ is any matrix satisfying $W_t^i(W_t^i)^g W_t^i = W_t^i$. Such a matrix is referred to as a generalized $(1)$-inverse \dfknote{would be good to cite a reference here since most folks will not know this term} of $W_t^i$. The Moore-Penrose Pseudo-Inverse is one example of such a matrix. 

% We have then 
% \begin{equation}
%     \label{eq:gpolicy_in_terms_of_others}
%     \begin{aligned}
%     \hat{\pi}_t^i(x_t) &:= [(W_t^i)^{g}]_{1:m^i}(-W_t^{-i}u_t^{-i} + Y_t x_t + y_t) \\
%     &:= \begin{bmatrix} \tilde{W}_t^{i,1} & \hdots & \tilde{W}_t^{i,i-1} & \tilde{W}_t^{i,i+1} & \hdots & \tilde{W}_t^{i,N} \end{bmatrix} u_t^{-i} + \tilde{Y}_t^i x_t + \tilde{y}_t^i
%     \end{aligned}
% \end{equation}

% As before, there exist controls $u_t^i$ jointly satisfying \cref{eq:private_kkt} if 
% \begin{equation}
%     \label{eq:nash_joint_policies}
%      \begin{bmatrix}  I & -\tilde{W}_t^{1,2} & \hdots & \hdots & -\tilde{W}_t^{1,N} \\
%      -\tilde{W}_t^{2,1} & I & \ddots  & \ddots & \vdots \\
%      \vdots & \ddots & \ddots &\ddots &\vdots \\
%      \vdots & \ddots & \ddots  & I & -\tilde{W}_t^{N-1,N} \\
%      -\tilde{W}_{t}^{N,1} & \hdots & \hdots & -\tilde{W}_t^{N,N-1}  & I
%     \end{bmatrix} u_t = 
%     \begin{bmatrix} \tilde{Y}_t^1 \\ \vdots \\ \tilde{Y}_t^N \end{bmatrix} x_t + \begin{bmatrix} \tilde{y}_t^i \\ \vdots \\ \tilde{y}_t^N \end{bmatrix}
% \end{equation}

% If the matrix in the left-hand-side of \cref{eq:nash_joint_policies} is singular, then the game is ill-posed and no equilibrium exists. \fnote{Double check and prove this. I think this matrix should always be full rank}. 





% \begin{equation}
% \hat{\pi}_T(x_T) = [W^g_T]_{1:m}(Y_T x_T + w_T) 
% \end{equation}
% satisfies condition \cref{eq:generalized_1_inverse_condition} by definition. However, the conditions \cref{eq:player_i_feasible,eq:player_i_g_inverse} prevent synthesizing the policies through use of, for example, the Moore-Penrose Pseudo-Inverse of $W_T$. 


% \begin{subequations}
% \label{eq:gn_problem_t}
% \begin{alignat}{3}
%     \pi_t^i(x_t) := \tilde{u}^i_t = \underset{u_t^i }{\textrm{\emph{arg}}} \underset{\substack{u_{t:T}^i,\\
%     \tilde{u}^{-i}_{t+1:T},\\
%     x_{t+1:T+1}}}{\textrm{\emph{min}}}\ 
%         &\sum_{s=t}^T l_s^i(x_s,u_s^i, \tilde{u}_s^{-i}) + l_{T+1}^i(x_{T+1}) 
%     \\
%     \textrm{\emph{s.t.}} \ \ \ \ 
%      (u_s^i,\tilde{u}^{-i}_s) &= \pi_s(x_s), \ s\in\mathbf{T_{t+1}} \label{eq:policy_of_other_controls}\\
%     x_{s+1} &= f(x_s,u_t^i, \tilde{u}_s^{-i}), \ s\in\mathbf{T_t} \\
%      u_t^i &\in \underset{u_{t}^i}{\text{\emph{argmin}}} \left\lVert e_t^i(x_t,u^i_t,\tilde{u}_t^{-i},...,x_{T+1}) \right\rVert  \label{eq:argmin_t}
%     % & 0 = h_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     % & 0 \leq g_s^i(x_s,u_t^i, \tilde{u}_s^{-i}), &&s\in\mathbf{T_t} \\
%     % & 0 = h^i_{T+1}(x_{T+1}) \\
%     % & 0 \leq g^i_{T+1}(x_{T+1})
% \end{alignat}
% \end{subequations}

% The constraints \cref{eq:argmin_T,eq:argmin_t} are expressed in this form to ensure that the problems defined are always feasible. For $t\in\mathbf{T}$, if $x_t$ and $\tilde{u}_t^{-i}$ are such that the minimization in \cref{eq:policies} is finite, then minimization appearing in \cref{eq:argmin_T,eq:argmin_t} attains a value of $0$. In this setting, the constraints \cref{eq:argmin_T,eq:argmin_t} are treated as hard constraints, and 
% The optimal values of $u_t^i$ are those which, among constraint-feasible controls, minimize the cost functional for player $i$.  If the minimization in these constraints does not attain a value of 0, then the minimum in \cref{eq:policies} is infinite, and any choice of $u_t^i$ is optimal for \cref{eq:policies}. In this setting, we arbitrarily choose $u_t^i$ to be that which is defined by \cref{eq:gn_problem_T,eq:gn_problem_t}. 

% Notably missing is the constraint $u_s^i = \pi_s^i(x_s)$, $s\in\mathbf{T_{t+1}}$, which is omitted due to redundancy. This redundancy be seen by equivalently expressing \cref{eq:gn_problem_t} as the following.

% \begin{subequations}
% \label{eq:gn_problem_t_alternate}
% \begin{alignat}{3}
%     \pi_t^i(x_t) := \tilde{u}^i_t = \underset{u_t^i }{\textrm{argmin}}\Bigg[
%     % \underset{\substack{u_{t:T}^i,\\
%     % \tilde{u}^{-i}_{t+1:T},\\
%     % x_{t+1:T+1}}}{\textrm{min}}\ 
%         &\ l_t^i(x_t,u_t^i,\tilde{u}_t^{-i}) +  \underset{\substack{u_{t+1:T}^i,\\
%     \tilde{u}^{-i}_{t+1:T},\\
%     x_{t+2:T+1}}}{\textrm{min}}\ \sum_{s=t+1}^T l_s^i(x_s,u_s^i, \tilde{u}_s^{-i}) + l_{T+1}^i(x_{T+1}) \Bigg]
%     \\
%     \textrm{s.t.} \ \ \ \ 
%      \tilde{u}^{-i}_s &= \pi^{-i}_s(x_s), \ s\in\mathbf{T_{t+1}} \\
%     x_{s+1} &= f(x_s,u_t^i, \tilde{u}_s^{-i}), \ s\in\mathbf{T_t} \\
%     \begin{bmatrix} u_{t+1}^i \\ \vdots  \\ u_{T}^i  \end{bmatrix} &\in \underset{u_{t+1:T}^i}{\text{argmin}} \sum_{s=t+1}^T\left\lVert e_s^i(x_s,u^i_s,\tilde{u}_s^{-i}) \right\rVert + \left\lVert e_{T+1}^i(x_{T+1}) \right\rVert \\
%     u_{t}^i  &\in \underset{u_{t}^i}{\text{argmin}} \sum_{s=t}^T\left\lVert e_s^i(x_s,u^i_s,\tilde{u}_s^{-i}) \right\rVert + \left\lVert e_{T+1}^i(x_{T+1}) \right\rVert
%     % \begin{bmatrix} u_{t+1}^i \\ \vdots  \\ u_{T}^i  \end{bmatrix} &\in \underset{u_{t+1:T}^i}{\text{argmin}} \left\lVert e_{t+1}^i(x_{t+1},u^i_{t+1},\tilde{u}_{t+1}^{-i},...,x_{T+1}) \right\rVert_2 \label{eq:argmin_tp1} \\
%     % u_t^i &\in \underset{u_{t}^i}{\text{argmin}} \left\lVert e_t^i(x_t,u^i_t,\tilde{u}_t^{-i},...,x_{T+1}) \right\rVert_2 \label{eq:argmin_only_t}
% \end{alignat}
% \end{subequations}

% For each player $i\in\mathbf{N}$, and $t\in\{1,...,T-1\}$, it can be seen that the optimization defined by \cref{eq:gn_problem_T,eq:gn_problem_t} for stages $t+1$ through $T$ for the same player $i$ are encapsulated within the problem \cref{eq:gn_problem_t} for stage $t$. 

% The purpose of redefining the policies in \cref{eq:policies} in terms of \cref{eq:gn_problem_T,eq:gn_problem_t} is to allow for the derivation of necessary conditions associated to a GFNE equilibrium trajectory. 

% At some iteration $k-1$ of \cref{alg:lq_ineq}, let $\mathbf{P}_{k-1} == 0$, and there exist at least one negative multiplier associated with an inequality constraint in the working set $\mathcal{W}_{k-1}$. Let $(t_m,i_m,j_m)$ be the index computed in \cref{line10} at this iteration, and $\mathcal{W}_k$ defined as in \cref{line12} by removing this index from the set $\mathcal{W}_{k-1}$. If the quadratic cost functional cross terms $R_t^{i,j,k} = 0, \ \forall j\neq i, k\neq i$, and the conditions in \cref{thm:sufficiency} hold for the problem \cref{eq:quadratic_cost_functional_active}, \cref{eq:linear_dynamics_active}, \cref{eq:linear_eq_constraints_active}, then $G_{x_{t_m}}^{i_m,j_m}x_{t_m} + G_{u_{t_m}}^{i_m,j_m}u_{t_m} + g_{t_m}^{i_m,j_m} \geq 0$ for all $\alpha \in [0,1]$, where $(x_{t_m}, u_{t_m})$ are the states and controls at stage $t_m$ of the game trajectory $\mathbf{X}_k + \alpha \mathbf{P}_k$.
% \end{theorem}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
